Friction Variability in Planar Pushing Data: Anisotropic Friction and Data-collection Bias

Friction plays a key role in manipulating objects. Most of what we do with our hands, and most of what robots do with their grippers, is based on the ability to control frictional forces. This paper aims to better understand the variability and predictability of planar friction. In particular, we focus on the analysis of a recent dataset on planar pushing by Yu et al. [1] devised to create a data-driven footprint of planar friction. We show in this paper how we can explain a significant fraction of the observed unconventional phenomena, e.g., stochasticity and multi-modality, by combining the effects of material non-homogeneity, anisotropy of friction and biases due to data collection dynamics, hinting that the variability is explainable but inevitable in practice. We introduce an anisotropic friction model and conduct simulation experiments comparing with more standard isotropic friction models. The anisotropic friction between object and supporting surface results in convergence of initial condition during the automated data collection. Numerical results confirm that the anisotropic friction model explains the bias in the dataset and the apparent stochasticity in the outcome of a push. The fact that the data collection process itself can originate biases in the collected datasets, resulting in deterioration of trained models, calls attention to the data collection dynamics.

==> dm-iros-journal-final <==
% Generated by IEEEtranN.bst, version: 1.13 (2008/09/30)
\begin{thebibliography}{21}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtranN.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem[Yu et~al.(2016)Yu, Bauza, Fazeli, and Rodriguez]{Yu2016MorePushing}
K.-T. Yu, M.~Bauza, N.~Fazeli, and A.~Rodriguez, ``{More than a Million Ways to
  Be Pushed: A High-Fidelity Experimental Data Set of Planar Pushing},'' in
  \emph{IEEE/RSJ Internatinonal Conference on Intelligent Robots and Systems
  (IROS)}, 2016.

\bibitem[Bauza and Rodriguez(2017)]{Bauza2017APushing}
M.~Bauza and A.~Rodriguez, ``{A Probabilistic Data-Driven Model for Planar
  Pushing},'' in \emph{IEEE International Conference on Robotics and Automation
  (ICRA)}, 2017.

\bibitem[Mason(1986)]{Mason1986MechanicsOperations}
M.~T. Mason, ``{Mechanics and Planning of Manipulator Pushing Operations},''
  \emph{The International Journal of Robotics Research}, vol.~5, no.~3, pp.
  53--71, 1986.

\bibitem[Peshkin and Sanderson(1988)]{Peshkin1988MotionWorkpiece}
M.~A. Peshkin and A.~C. Sanderson, ``{Motion of a pushed, sliding workpiece},''
  pp. 569--598, 1988.

\bibitem[Lynch et~al.(1992)Lynch, Maekawa, and
  Tanie]{Lynch1992ManipulationFeedback}
K.~Lynch, H.~Maekawa, and K.~Tanie, ``{Manipulation And Active Sensing By
  Pushing Using Tactile Feedback},'' \emph{Proceedings of the IEEE/RSJ
  International Conference on Intelligent Robots and Systems}, vol.~1, pp.
  416--421, 1992.

\bibitem[Jia and Erdmann(1999)]{Jia1999PoseContact}
Y.~B. Jia and M.~Erdmann, ``{Pose and motion from contact},''
  \emph{International Journal of Robotics Research}, vol.~18, no.~5, pp.
  466--490, 1999.

\bibitem[Liu(2011)]{Liu2011PushingModel}
H.~Liu, ``{Pushing With A Physics-Based Model},'' Ph.D. dissertation,
  Massachusetts Institute of Technology, 2011.

\bibitem[Lynch and Mason(1996)]{Lynch1996StablePlanning}
K.~M. Lynch and M.~T. Mason, ``{Stable Pushing: Mechanics, Controllability, and
  Planning},'' \emph{The International Journal of Robotics Research}, vol.~15,
  no.~6, pp. 533--556, 1996.

\bibitem[Behrens(2013)]{Behrens2013RoboticTechniques}
M.~J. Behrens, ``{Robotic Manipulation by Pushing at a Single Point with
  Constant Velocity : Modeling and Techniques},'' Ph.D. dissertation,
  University of Technology, Sydney, 2013.

\bibitem[Hogan and Rodriguez(2016)]{Hogan2016FeedbackDynamics}
F.~Hogan and A.~Rodriguez, ``{Feedback Control of the Pusher-Slider System: A
  Story of Hybrid and Underactuated Contact Dynamics},'' \emph{Workshop on
  Algorithmic Foundation of Robotics (WAFR)}, 2016.

\bibitem[Marone(1998)]{Marone1998TheCycle}
C.~Marone, ``{The effect of loading rate on static friction and the rate of
  fault healing during the earthquake cycle},'' \emph{Nature}, vol. 391, pp.
  69--72, 1998.

\bibitem[Mate et~al.(1987)Mate, McClelland, Erlandsson, and Chiang]{Mate1987}
C.~M. Mate, G.~M. McClelland, R.~Erlandsson, and S.~Chiang, ``{Atomic-scale
  friction of a tungsten tip on a graphite surface},'' \emph{Physical Review
  Letters}, vol.~59, no.~17, pp. 1942--1945, 1987.

\bibitem[Bylinskii et~al.(2015)Bylinskii, Gangloff, and
  Vuleti{\'{c}}]{Bylinskii2015}
A.~Bylinskii, D.~Gangloff, and V.~Vuleti{\'{c}}, ``{Tuning friction
  atom-by-atom in an ion-crystal simulator},'' \emph{Science}, vol. 348, no.
  6239, pp. 1115 -- 1118, jun 2015.

\bibitem[Yamashita et~al.(2015)Yamashita, Fukuyama, Mizoguchi, Takizawa, Xu,
  and Kawakata]{Yamashita2015}
F.~Yamashita, E.~Fukuyama, K.~Mizoguchi, S.~Takizawa, S.~Xu, and H.~Kawakata,
  ``{Scale dependence of rock friction at high work rate},'' \emph{Nature},
  vol. 528, no. 7581, pp. 254--257, dec 2015.

\bibitem[Zhou et~al.(2017)Zhou, Bagnell, and Mason]{Zhou2017AValidation}
J.~Zhou, J.~A. Bagnell, and M.~T. Mason, ``{A Fast Stochastic Contact Model for
  Planar Pushing and Grasping: Theory and Experimental Validation},'' in
  \emph{Robotics: Science and Systems (RSS)}, 2017.

\bibitem[Meri{\c{c}}li et~al.(2014)Meri{\c{c}}li, Veloso, and
  Akın]{Mericli2014Push-manipulationModels}
T.~Meri{\c{c}}li, M.~Veloso, and H.~L. Akın, ``{Push-manipulation of complex
  passive mobile objects using experimentally acquired motion models},''
  \emph{Autonomous Robots}, vol.~38, no.~3, pp. 317--329, 2014.

\bibitem[Salganicoff et~al.(1993)Salganicoff, Metta, Oddera, and
  Sandini]{Salganicoff1993MarcosSandini}
M.~Salganicoff, G.~Metta, A.~Oddera, and G.~Sandini, \emph{A vision-based
  learning method for pushing manipulation}.\hskip 1em plus 0.5em minus
  0.4em\relax University of Pennsylvania, 1993.

\bibitem[Lau et~al.(2011)Lau, Mitani, and Igarashi]{Lau2011AutomaticObjects}
M.~Lau, J.~Mitani, and T.~Igarashi, ``Automatic learning of pushing strategy
  for delivery of irregular-shaped objects,'' in \emph{Robotics and Automation
  (ICRA), 2011 IEEE International Conference on}.\hskip 1em plus 0.5em minus
  0.4em\relax IEEE, 2011, pp. 3733--3738.

\bibitem[Walker and Salisbury(2008)]{Walker2008PushingMaps}
S.~Walker and J.~K. Salisbury, ``{Pushing using learned manipulation maps},''
  \emph{Proceedings - IEEE International Conference on Robotics and
  Automation}, pp. 3808--3813, 2008.

\bibitem[Zhou et~al.(2016)Zhou, Paolini, Bagnell, and
  Mason]{Zhou2016AApplication}
J.~Zhou, R.~Paolini, J.~A. Bagnell, and M.~T. Mason, ``A convex polynomial
  force-motion model for planar sliding: Identification and application,'' in
  \emph{Robotics and Automation (ICRA), 2016 IEEE International Conference
  on}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2016, pp. 372--377.

\bibitem[Goyal et~al.(1991)Goyal, Ruina, and
  Papadopoulos]{Goyal1991PlanarFunction}
S.~Goyal, A.~Ruina, and J.~Papadopoulos, ``{Planar sliding with dry friction
  Part 1. Limit surface and moment function},'' \emph{Wear}, vol. 143, no.~2,
  pp. 307--330, 1991.

\end{thebibliography}

